Exoplanet System Kepler-2 with comparisons to Kepler-1 and 13

We have carried out an intensive study of photometric (Kepler Mission) and spectroscopic data on the system Kepler-2 (HAT-P-7A) using the dedicated software WinFitter. The mean individual data-point error of the normalized flux values for this system is 0.00015, leading to the model's specification for the mean reference flux to an accuracy of $\sim$0.5 ppm. This testifies to the remarkably high accuracy of the binned data-set, derived from over 1.8 million individual observations. Spectroscopic data are reported with the similarly high-accuracy radial velocity amplitude measure of $\sim$2 m s$^{-1}$. The analysis includes discussion of the fitting quality and model adequacy. Our derived absolute parameters for Kepler-2 are as follows: $M_p$ (Jupiter) 1.80 $\pm$ 0.13; $R_{\star}$ 1.46 $\pm 0.08 \times 10^6$ km; $R_p$ 1.15 $\pm 0.07 \times 10^5$ km. These values imply somewhat larger and less condensed bodies than previously catalogued, but within reasonable error estimates of such literature parameters. We find also tidal, reflection and Doppler effect parameters, showing that the optimal model specification differs slightly from a `cleaned' model that reduces the standard deviation of the $\sim$3600 binned light curve points to less than 0.9 ppm. We consider these slight differences, making comparisons with the hot-jupiter systems Kepler-1 (TrES-2) and 13.

==> bib.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Albrecht}{2012}]{alb} % %
Albrecht, S., et al.\ (12 authors), 2012, ApJ, 757, 18

\bibitem[\protect\citeauthoryear{Alonso}{2004}]{alo} % %
Alonso, R., et al.\ (11 authors), 2004, ApJ, 613, L153

\bibitem[\protect\citeauthoryear{Angerhausen}{2015}]{ang} % %
Angerhausen, D., DeLarme, E. and Morse, J. A., 2015, PASP, 127, 1113

\bibitem[\protect\citeauthoryear{Armstrong}{2016}]{arm} % %
Armstrong, D.J., et al.\ (5 authors), 2016, Nature Astronomy, 1, 0004

\bibitem[\protect\citeauthoryear{Barclay}{2015}]{ba2} % %
Barclay, T., et al.\ (7 authors), 2015, ApJ, 800, 46

\bibitem[\protect\citeauthoryear{Barnes}{2011}]{brn} % %
Barnes, J. W., Linscott, E. and Shporer, A., 2011, ApJS, 197, 10

\bibitem[\protect\citeauthoryear{Batalha}{2013}]{bat} % %
Batalha, N.M., et al.\ (75 authors), 2013, ApJS, 204, 24

\bibitem[\protect\citeauthoryear{Benomar}{2014}]{ben} % %
Benomar, O., et al.\ (3 authors), 2014, PASJ, 66, 94

\bibitem[\protect\citeauthoryear{Berdyugina}{2002}]{ber} % %
Berdyugina, S. V., 2002, AN, 323, 192-195

\bibitem[\protect\citeauthoryear{Borucki}{2003}]{bo1} % %
Borucki, W.J., et al.\ (14 authors), 2003, in {\em Scientific Frontiers in Research on Extrasolar Planets}, Eds.\ 
D.\ Deming and S.\ Seager, ASP Conf.\ Ser.\, 294, 427

\bibitem[\protect\citeauthoryear{Borucki}{2009}]{bo2} % %
Borucki, W.J., et al.\ (24 authors), 2009, Sci, 325, 709

\bibitem[\protect\citeauthoryear{Borucki}{2011}]{bo3} % %
Borucki, W.J., et al.\ (69 authors), 2011, ApJ, 736, 19

\bibitem[\protect\citeauthoryear{Boue}{2013}]{bou} % %
Bou\'{e}, G., et al.\ (4 authors), 2013, A\&A, 550, A53

\bibitem[\protect\citeauthoryear{Brown}{2011}]{br1} % %
Brown, T.M., et al.\ (3 authors), 2011, AJ, 142, 112

\bibitem[\protect\citeauthoryear{Brown}{2017}]{br2} % %
Brown, D. J. A., et al.\ (14 authors), 2017, MNRAS, 464, 810-839

\bibitem[\protect\citeauthoryear{Budding}{2007}]{bu1} % %
Budding, E. and Demircan, O., 2007, {\em Introduction to Astronomical Photometry}, CUP

\bibitem[\protect\citeauthoryear{Budding}{2016}]{bu2} % %
Budding, E., et al. (5 authors), 2016, Ap{\&}SS, 361, 346

\bibitem[\protect\citeauthoryear{Budding}{2018}]{bu3} % %
Budding, E., P\"{u}sk\"{u}ll\"{u}, \c{C}. and Rhodes, M.D., 2018, Ap{\&}SS, 363, 60

\bibitem[\protect\citeauthoryear{Butler}{1996}]{but} % %
Butler, R. P., et al. (5 authors), 1996, PASP, 108, 500

\bibitem[\protect\citeauthoryear{Butler}{2006}]{btl} % %
Butler, R. P, et al. (10 authors), 2006, ApJ, 646, 505-522

\bibitem[\protect\citeauthoryear{Catling}{2017}]{cat} % %
Catling, D.C. and Kasting, J.F., 2017, Atmospheric Evolution on Inhabited and Lifeless Worlds

\bibitem[\protect\citeauthoryear{Christensen-Dalsgaard}{2010}]{chd} % %
Christensen-Dalsgaard, J., et al. \ (9 authors), 2010, ApJL, 2010, 713, L164-L168

\bibitem[\protect\citeauthoryear{Christian}{2010}]{chr} % %
Christian, D.J. and Lund, M.B., 2010, AAS-DPS, 42, 27

\bibitem[\protect\citeauthoryear{Daemgen}{2009}]{dae} % %
Daemgen, S., et al. (6 authors), 2009, A{\&}A 498, 567

\bibitem[\protect\citeauthoryear{Dotson}{2019}]{dot} % %
Dotson, J., 2019, \emph{https://keplerscience.arc.nasa.gov}

\bibitem[\protect\citeauthoryear{Esteves}{2013}]{es1} % %
Esteves, L. J., De Mooij, E. J. W. and Jayawardhana, R., 2013, ApJ, 772, 51

\bibitem[\protect\citeauthoryear{Esteves}{2015}]{es2} % %
Esteves, L. J., De Mooij, E. J. W. and Jayawardhana, R., 2015, ApJ, 804, 150

\bibitem[\protect\citeauthoryear{Faedi }{2013}]{fai} % %
Faedi, F., et al. \ (9 authors), 2013, MNRAS, 433, 2097-2106

\bibitem[\protect\citeauthoryear{Faigler}{2013}]{fa1} % %
Faigler, S., et al.\ (4 authors), 2013, ApJ, 771, 26

\bibitem[\protect\citeauthoryear{Faigler}{2015}]{fa2} % %
Faigler, S. and Mazeh, T., 2015, ApJ, 800, 73

\bibitem[\protect\citeauthoryear{Guzik}{2014}]{guz} % %
Guzik, J. A.; Chaplin, W. J.; Handler, G. and Pigulski, A. (Eds.), 2014, Precision Asteroseismology, 301

\bibitem[\protect\citeauthoryear{Hansen}{2007}]{han} % %
Hansen, B.M.S. and Barman, T., 2007, ApJ, 671, 861

\bibitem[\protect\citeauthoryear{Hirano}{2011}]{hir} % %
Hirano, T., et al. (6 authors), 2011, ApJ, 742, 69

\bibitem[\protect\citeauthoryear{Hosokawa}{1958}]{hos} % %
Hosokawa, Y., 1958, PASJ 10, 120

\bibitem[\protect\citeauthoryear{Howard}{2009}]{how} % %
Howard, A.\ (and SIM Team), 2009, BAAS, 214, 750

\bibitem[\protect\citeauthoryear{Johnson}{2014}]{joh} % %
Johnson, M.C., et al.\ (5 authors), 2014, ApJ, 790, 30

\bibitem[\protect\citeauthoryear{Kipping}{2011}]{kip} % %
Kipping, D.M. and Spiegel, D.S., 2011, MNRAS, 417, 88

\bibitem[\protect\citeauthoryear{Kirbiyik}{1976}]{kir} % %
K{\i}rb{\i}y{\i}k, H. and Smith, R. C., 1976, MNRAS, 176, 103-129

\bibitem[\protect\citeauthoryear{Kopal}{1959}]{kop} %
Kopal, Z., 1959, {\em Close Binary Systems}, Chapman \& Hall, London \& New York

\bibitem[\protect\citeauthoryear{Kourganoff}{1952}]{kur} % %
Kourganoff, V., 1952, {\em Basic methods in transfer problems; radiative equilibrium and neutron diffusion}, Oxford, Clarendon Press

\bibitem[\protect\citeauthoryear{Libralato}{2016}]{lib} % %
Libralato, M., et al.\ (9 authors), 2016, MNRAS, 463, 1780-1796

\bibitem[\protect\citeauthoryear{Lillo-Box}{2014}]{li1} % %
Lillo-Box, J., et al.\ (8 authors), 2014, A\&A, 568, L1

\bibitem[\protect\citeauthoryear{Lillo-Box}{2016}]{li2} % %
Lillo-Box, J., et al.\ (4 authors), 2016, A\&A, 592, A32

\bibitem[\protect\citeauthoryear{Lund}{2014}]{lun} % %
Lund, M.N.., et al.\ (14 authors), 2014, A\&A, 570, A54

\bibitem[\protect\citeauthoryear{Madhusudhan}{2017}]{mad} % %
Madhusudhan, N., et al.\ (3 authors), 2017, MNRAS, 469, 4102-4115

\bibitem[\protect\citeauthoryear{Masuda}{2015}]{mas} % %
Masuda, K., 2015, ApJ, 805, 28

\bibitem[\protect\citeauthoryear{Mazeh}{2012}]{maz} % %
Mazeh, T., et al.\ (4 authors), 2012, A\&A, 541, A56

\bibitem[\protect\citeauthoryear{McNally}{1965}]{mcn} % %
McNally, D., 1965, Obs, 85, 166-169

\bibitem[\protect\citeauthoryear{Mislis}{2012}]{mis} % %
Mislis, D. and Hodgkin, S., 2012, MNRAS, 422, 1512-1517

\bibitem[\protect\citeauthoryear{Morris}{2013}]{mor} % %
Morris, C. K., et al.\ (3 authors), 2013, AGU Fall Meeting Abstracts, H13E-1389

\bibitem[\protect\citeauthoryear{Narita}{2009}]{nar} % %
Narita, N., et al.\ (3 authors), 2009, PASJ, 61, L35-L40

\bibitem[\protect\citeauthoryear{Neuhauser}{2011}]{neu} % %
Neuh\"{a}user, R., et al.\ (82 authors), 2011, AN, 332, 547

\bibitem[\protect\citeauthoryear{Nielsen}{2013}]{nie} % %
Nielsen, M. B., et al.\ (3 authors), 2013, Progress in Physics of the Sun and Stars: A New Era in Helio- and Asteroseismology, 479, 137

\bibitem[\protect\citeauthoryear{O'Donovan}{2006}]{odo} % %
O'Donovan, F.T., et al.\ (19 authors), 2006, ApJ, 651, L61

\bibitem[\protect\citeauthoryear{Oshagh}{2015}]{osg} % %
Oshagh, M., et al.\ (6 authors), 2015, A\&A, 583, L1

\bibitem[\protect\citeauthoryear{Pal}{2008}]{pal} % %
P\'{a}l, A., et al.\ (16 authors), 2008, ApJ, 680, 1450-1456

\bibitem[\protect\citeauthoryear{Rhodes}{2014}]{rh1} % %
Rhodes, M.D. and Budding, E., 2014, Ap\&SS, 351, 451-471

\bibitem[\protect\citeauthoryear{Rhodes}{2019}]{rh2} % %
Rhodes, M.D, 2019, \ {\em WinFitter v.6 User Manual}

\bibitem[\protect\citeauthoryear{Rowe}{2011}]{row} % %
Rowe, J., et al.\ (9 authors), 2011, AAS Meeting Abstracts 218, 43, 211

\bibitem[\protect\citeauthoryear{Safronov}{1972}]{saf} % %
Safronov, V.S., 1972, IAUSymp.\ 45, Reidel, Dordrecht, p 329

\bibitem[\protect\citeauthoryear{Santerne}{2012}]{san} % %
Santerne, A., et al.\ (9 authors), 2012, A\&A, 544, L12

\bibitem[\protect\citeauthoryear{Schrijver}{2001}]{sch} % %
Schrijver, C. J. and Title, A. M., 2001, ApJ, 551, 1099-1106

\bibitem[\protect\citeauthoryear{Shporer}{2012}]{sh1} % %
Shporer, A., et al.\ (3 authors), 2012, NewA, 17, 309-315

\bibitem[\protect\citeauthoryear{Shporer}{2014}]{sh2} % %
Shporer, A., et al.\ (9 authors), 2014, AJ, 142, 195

\bibitem[\protect\citeauthoryear{Shibahashi}{2013}]{shi} % %
Shibahashi, H. and Lynas-Gray, A. E. (Eds.), 2013, Progress in Physics of the Sun and Stars: A New Era in Helio- and Asteroseismology, 479

\bibitem[\protect\citeauthoryear{Smith}{2012}]{smi} % %
Smith, J.C.\ et al.\ (11 authors) 2012, PASP, 124, 1000

\bibitem[\protect\citeauthoryear{Sozzetti}{2007}]{soz} % %
Sozzetti, A., et al. (7 authors), F.T., 2007, ApJ, 664, 1190

\bibitem[\protect\citeauthoryear{Stumpe}{2012}]{stu} % %
Stumpe, M.C.\ et al.\ (11 authors), 2012, PASP, 124, 985

\bibitem[\protect\citeauthoryear{Twicken}{2010}]{twi} % %
Twicken J.D., et al. (5 authors), 2010, SPIE Conf.\ Ser.\, 7740, p77401-U-1

\bibitem[\protect\citeauthoryear{van Eylen}{2013}]{van} % %
van Eylen, V., et al. (4 authors), 2013, ApJL, 774, L19

\bibitem[\protect\citeauthoryear{vonParis}{2016}]{voP} % %
von Paris, P., et al. \ (4 authors), 2016, A\&A, 589, A52

\bibitem[\protect\citeauthoryear{Welsh}{2010}]{wel} % %
Welsh, W.F., et al.\ (7 authors), 2010, American Astronomical Society Meeting Abstracts 215, 42, 318

\bibitem[\protect\citeauthoryear{Winn}{2009}]{win} % %
Winn, J.N., et al.\ (6 authors), 2009, ApJL, 703, L99-L103

\bibitem[\protect\citeauthoryear{Wong}{2016}]{wng} % %
Wong, I., et al.\ (17 authors), 2016, ApJ, 823, 122

\bibitem[\protect\citeauthoryear{Zeilik}{1988}]{zei} % %
Zeilik, M., et al.\ (3 authors), 1988, ApJ, 332, 293-298

\end{thebibliography} 
